Passive advection of percolation process: Two-loop approximation

The paradigmatic model of the directed percolation process is studied near its second order phase transition between an absorbing and an active state. The model is first expressed in a form of Langevin equation and later rewritten into a field-theoretic formulation. The ensuing response functional is then analyzed employing Feynman diagrammatic technique and perturbative renormalization group method. Percolation process is assumed to occur in external velocity field, which has an additional effect on spreading properties. Kraichnan rapid change ensemble is used for generation of velocity fluctuations. The structure of the fixed points structure is obtained within the two-loop approximation.

==> biblio_help.tex <==
%
%    SORT CITATIONS IN THE ARTICLE ACCORDING FIRST APPEARANCE - DO AT THE VERY END OF PREPARATIONS
%
\begin{thebibliography}{99}
 \bibitem{Hin06} H.~Hinrichsen, Physica A {\bf 369}, 1 (2006).
 \bibitem{Stauffer} D.~Stauffer, A.~Aharony, {\it Introduction to Percolation Theory}
     (Taylor and Francis, London, 1992).
 \bibitem{HHL08} M.~Henkel, H.~Hinrichsen, S.~L{\"u}beck, 
     {\it Non-equilibrium phase transitions: Volume 1 – Absorbing phase transitions}, 
     (Springer, Dordrecht, 2008).
 \bibitem{Schlogl} F.~Schl\"ogl, Z. Phys. {\bf 253}, 147 (1972).
 \bibitem{Grassberger82} P.~Grassberger, Z. Phys. B: Condens. Matter {\bf 47}, 365 (1982).
 \bibitem{Gribov} V.~N.~Gribov, Sov. Phys. JETP {\bf 26}, 414 (1968).    
 \bibitem{Cardy} J. L. Cardy and R. L. Sugar, \emph{ J. Phys. A} {\bf 13}, L423–L427, (1980).
 \bibitem{Hinrichsen} H.~Hinrichsen, J. Stat. Mech.: Theor. Exp. P07066 (2007).
 \bibitem{Janssen81} H.~K.~Janssen, Z. Phys. B: Condens. Matter {\bf 42}, 151 (1981).
 \bibitem{Janssen96} H.~K.~Janssen, Phys. Rev. E {\bf 55}, 6253 (1997).
 \bibitem{RRR03} P.~Rupp, R.~Richter, I.~Rehberg, Phys. Rev. E {\bf 67}, 036209 (2003).
 \bibitem{TKCS07} K.~A.~Takeuchi, M.~Kuroda, H.~Chat, M.~Sano, Phys. Rev. Lett. {\bf 99}, 234503 (2007).
 \bibitem{FGV01} G.~Falkovich, K.~Gaw\c{e}dzki, M.~Vergassola, Rev. Mod. Phys. {\bf 73}, 913 (2001). 
 \bibitem{Landau_fluid} L.~D.~Landau and E.~M.~Lifshitz, {\it Fluid Mechanics} (Pergamon Press, 1959).
 \bibitem{Frisch} U.~Frisch, {\it Turbulence: The Legacy of A. N. Kolmogorov} (Cambridge University Press, Cambridge, 1995). 
 \bibitem{Monin} A.~S.~Monin and A.~M.~Yaglom, {\it Statistical Fluid Mechanics:Vol 2}
    (MIT Press, Cambridge, 1975). 
 \bibitem{Ant99} N.~V.~Antonov, Phys. Rev. E {\bf 60}, 6691 (1999).
 \bibitem{Benzi09} R.~Benzi and D.~R.Nelson", Physica D {\bf 238}, 2003 (2009).
 \bibitem{Pig12} S.~Pigolotti and R.~Benzi and M.~H.~Jensen and D.~R.~Nelson, 
    Phys. Rev. Lett. {\bf 108}, 128102 (2012).
 \bibitem{Volk14} R.~Volk and C.~Mauger and M.~Bourgoin and C.~Cottin-Bizonne
	      and C.~Ybert and F.~Raynal, Phys. Rev. E {\bf 90}, 013027 (2014).
 \bibitem{depietro15} M.~De~Pietro and M.~A.~T.~van~Hinsberg and L.~Biferale and
	      H.~J.~H.~Clercx and P.~Perlekar and F.~Toschi, Phys. Rev. E {\bf 91}, 053002 (2015).
 \bibitem{Ant00} N.~V.~Antonov, Physica D {\bf 144}, 370 (2000).
 \bibitem{AntKap08} N.~V.~Antonov, V.~I.~Iglovikov, A.~S.~Kapustin, J. Phys. A: Math. Theor. {\bf 42}, 135001 (2008).
 \bibitem{AntKap10} N.~V.~Antonov, A.~S.~Kapustin, J. Phys. A: Math. Theor. {\bf 43}, 405001 (2010).
 \bibitem{Ant11} N.~V.~Antonov, A.~S.~Kapustin, A.~V.~Malyshev, Theor. Math. Phys. {\bf 169}, 1470 (2011).
 \bibitem{DP13} M.~Dan\v{c}o, M.~Hnati\v{c}, T.~Lu\v{c}ivjansk\'{y} and L.~Mi\v{z}i\v{s}in, Theor. Math. Phys. {\bf 176}, 898 (2013).
 \bibitem{Vasiliev} A.~N.~Vasil'ev, {\it The Field Theoretic Renormalization Group in Critical Behavior Theory and Stochastic Dynamics}
 \bibitem{JanTau04} H.~K.~Janssen, U.~C.~T{\"a}uber, Ann. Phys. {\bf 315}, 147 (2004).
 \bibitem{Doi} M.~Doi, J. Phys. A {\bf 9}, 1465 (1976); {\it ibid.} {\bf 9}, 1479 (1976).        
 \bibitem{Janssen76} H.~K.~Janssen, Z. Phys. B: Condens. Matter {\bf 23}, 377 (1976).
 \bibitem{deDom76} C.~De~Dominicis, J. Phys. Colloq. France {\bf 37}, C1-247 (1976).
 \bibitem{Janssen79} H.~K.~Janssen, {\it Dynamical Critical Phenomena and Related Topics},
    Lect. Notes Phys. {\bf 104}, (Springer, Heidelberg, 1979).
 \bibitem{Zinn} J.~Zinn-Justin, \textit{Quantum Field Theory and Critical Phenomena} (Oxford University Press, Oxford, 1989).   
 \bibitem{AdzAnt98} L.~Ts.~Adzhemyan, N.~V.~Antonov, Phys. Rev. E {\bf 58}, 7381 (1998).   
 \bibitem{Amit} D. J. Amit and V. Mart\'in-Mayor, {\it Field Theory, the Renormalization Group and Critical Phenomena}
 (World Scientific, Singapore, 2005). 
 \bibitem{Tauber2014} U.~T{\"a}uber, {\it Critical Dynamics: A Field Theory Approach to Equilibrium
 	      and Non-Equilibrium Scaling Behavior}
 	      (Cambridge University Press , New York, 2014).
 \bibitem{AAK94} L.~Ts. Adzhemyan, N.~V.~Antonov, T.~L.~Kim, Theor. Math. Phys. {\bf 100}, 1086 (1994).
 \bibitem{ABG96} N.~V.~Antonov, S.~V.~Borisenok, V.~I.~Girina, Theor. Math. Phys. {\bf 106}, 75 (1996).
 \bibitem{AV97} N.~V.~Antonov, A.~N.~Vasil'ev, Theor. Math. Phys. {\bf 110}, 97 (1997).
 \bibitem{FNS} D.~Forster, D.~R.~Nelson, M.~J.~Stephen, Phys. Rev. A {\bf 16}, 732 (1977).
 \bibitem{HH00} M.~Hnatich, J.~Honkonen, Phys. Rev. E {\bf 61}, 3904 (2000).
 \bibitem{HonKar88} J.~Honkonen and E.~Karjalainen, J. Phys. A: Math. Gen. {\bf 21}, 4217 (1988). 
 \bibitem{GV99} K.~Gaw{\c{e}}dzki, M.~Vergasssola, Physica D {\bf 138}, 63 (1999).
\end{thebibliography}
